Assessing the Role of Datasets in the Generalization of Motion Deblurring Methods to Real Images

Successfully training end-to-end deep networks for real motion deblurring requires datasets of sharp/blurred image pairs that are realistic and diverse enough to achieve generalization to real blurred images. Obtaining such datasets remains a challenging task. In this paper, we first review the limitations of existing deblurring benchmark datasets and analyze the underlying causes for deblurring networks' lack of generalization to blurry images in the wild. Based on this analysis, we propose an efficient procedural methodology to generate sharp/blurred image pairs based on a simple yet effective model. This allows for generating virtually unlimited diverse training pairs mimicking realistic blur properties. We demonstrate the effectiveness of the proposed dataset by training existing deblurring architectures on the simulated pairs and performing cross-dataset evaluation on three standard datasets of real blurred images. When training with the proposed method, we observed superior generalization performance for the ultimate task of deblurring real motion-blurred photos of dynamic scenes.

==> about_CRF.tex <==
\subsection{What is CRF?}
The Camera Response Function (CRF) describes the relationship between the radiant energy the image sensor receives and the intensities observed in the output image. In practice, the majority of cameras have nonlinear CRFs \cite{grossberg2004modeling}, which arise from a combination of various internal camera processes. These processes encompass operations such as analog-digital conversion within the image sensor, white balance adjustment, gamma correction that compress a wide range of irradiance values within a fixed range of measurable image intensity to emulate the response of the human visual system, or the tone mapping employed to create diverse aesthetic effects.  

\subsection{Why CRF is important?}

Calibration of a camera response is crucial in many computer vision tasks. Examples of such tasks include image mosaicing, where multiple images must be flawlessly coupled, and high dynamic range imaging, where images of multiple exposures are used to produce images with greater dynamic ranges. 

According to \cite{sharma2020estimation}, CRF estimation is used for shape from shading [ 4], [5 ], color constancy [ 6], [7 ], photometric stereo [8 ], [9 ], specular removal [10], shadow removal [ 11], low-light image enhancement [12]

\subsection{CRF on deblurring}

The CRF influence in deblurring performance has been studied in depth by \cite{tai2013nonlinear} before the \textit{deep learning} era, but it has been chiefly disregarded recently.    

\subsection{How is CRF modeled?}
The Empirical Model of Response (EMoR) proposed by \cite{grossberg2004modeling} is the most widely used among the CRF models.  The EMoR describes a CRF by a linear combination of eigenvectors generated by applying Principal Component Analysis (PCA) on 201 real-world CRFs known as the Database of Response Function (DoRF). 

Polynomial and gamma curves are the other popular CRF representation models. Among the deblurring community, modeling the CRF as a gamma function is the default, probably because it was used in the pioneering work of Fergust, and used to generate the widely used GoPro dataset \cite{Nah_2017_CVPR}. Recently,  \cite{rim_2022_ECCV} used a polynomial curve to estimate the CRF.

\subsection{CRF estimation}

In the early approaches of CRF estimation, many methods relied on a sequence of images of the same scene taken with different exposure times [ 13], [ 14 ], [ 15 ] or varying illumination [8 ], [3]. In addition to requiring multiple images, these methods also assume that the camera position is fixed. Some other methods [ 23], [ 24 ], [ 25 ], [ 26 ], [27 ] have relaxed the fixed camera condition by performing image alignment. To improve the practicality, some recent methods utilize a single image. This, however, is considerably more challenging than using multiple images.

According to \cite{sharma2020estimation}, most existing methods for CRF estimation from a single image fail to handle general real images. This is because the methods require additional constraints that, in practice, may not hold. Matsushita and Lin [16 ] proposed a method based on the observation that the noise distribution is symmetric in the irradiance domain, but due to the non-linear CRF; it becomes asymmetric in the intensity domain. However, this method does not work well if there is insufficient data for generating the noise profile.  EdgeCRF [1] is based on the property that pixels around color boundaries in the camera irradiance form linear distributions in the RGB space. However, due to the non-linear CRF, the pixel distributions become non-linear for the intensity image in the RGB space. Thus the CRF is recovered by finding a CRF model that can linearise the distributions with minimum error. Later, the method is extended to work on grayscale images [28]. The ideas of these two methods are elegant, yet unfortunately, they are prone to suffer from noise that is commonly present in real images.
Unfortunately, the noise in many natural images [ 17] severely affects the methods \cite{sharma2020estimation}.  More recently, \cite{li2017crf} [2 ] proposed a network to estimate the CRF from a single image by predicting 11 coefficients of the basis functions model [ 20 ], for which they use the 201 CRFs from [20 ] during training.  However, it suffers from the generalization problem, which means it can only work effectively for CRFs represented in the training data.  To address these problems, \cite{sharma2020estimation} introduces a non-deep-learning method using prediction consistency and gradual refinement. Apparently, their generalization performance is better than CRFNet \cite{li2017crf}, making it more practically applicable for CRF estimation for general real images. In work cited by \cite{ng2007using}, a CRF estimation method for a single-channel image is proposed by assuming that non-linear transformation of image irradiance by a gamma curve, introduces correlated harmonics, which can be measured by the magnitude of bicoherence (third-order moment spectra) [3]. However, the method is limited to using the gamma curve CRF model, which is known to be insufficient for real-world CRF’s.


There is no code available.   

CRF estimation on blurry images is even more challenging since blur alters the assumptions made on edges and noise. \cite{tai2013nonlinear} propose a method to estimate the CRF, assuming the PSF is known, and also a blind estimation method. There is no code available.   


==> kernels_simulation.tex <==
\noindent\textbf{Kernels Simulation} \cite{chakrabarti2016neural} generated synthetic motion kernels by randomly sampling six points in a limited size grid, fitting a spline through these points, and setting the kernel values at each pixel on this spline to a value sampled from a sharp Gaussian. An adaptation of this method has been applied by \cite{kaufman2020deblurring}.

To generate random motion kernels~\cite{delbracio2015removing} propose a camera-shake kernel generator based on physiological hand tremor data~\cite{gavant2011physiological}. The shape and size of the motion blur kernel are control by a single parameter, the exposure time. Schmidt \etal~\cite{schmidt2015cascades} propose to sample random 3D trajectories using a simple linear motion model and then to project and rasterize the obtained trajectories to random square kernels of varying sizes. This method was later used by~\cite{rim_2020_ECCV} and \cite{lai2016comparative} to synthesize uniformly blurry images. \cite{lai2016comparative} also incorporates 6D camera trajectories by using a cellphone with inertial sensors (gyroscope and accelerometer) and construct a collection of spatially varying blur kernels by assuming constant depth scenes. 

To deal with the inherent phase ambiguity~\cite{chakrabarti2016neural} proposes a ``canonical'' translation by centering them so that each kernel’s center of mass is located at the center of the window. This strategy was also confirmed as useful by~\cite{rim_2020_ECCV}.\\

